A Bayesian Nonparametric Method to Adjust for Unmeasured Confounding with Negative Controls

Unmeasured confounding bias threatens the validity of observational studies. While sensitivity analyses and study designs have been proposed to address this issue, they often overlook the growing availability of auxiliary data. Using negative controls from these data is a promising new approach to reduce unmeasured confounding bias. In this article, we develop a Bayesian nonparametric method to estimate a causal exposure-response function (CERF) leveraging information from negative controls to adjust for unmeasured confounding. We model the CERF as a mixture of linear models. This strategy captures the potential nonlinear shape of CERFs while maintaining computational efficiency, and it leverages closed-form results that hold under the linear model assumption. We assess the performance of our method through simulation studies. We found that the proposed method can recover the true shape of the CERF in the presence of unmeasured confounding under assumptions. To show the practical utility of our approach, we apply it to adjust for a possible unmeasured confounder when evaluating the relationship between long-term exposure to ambient $PM_{2.5}$ and cardiovascular hospitalization rates among the elderly in the continental US. We implement our estimation procedure in open-source software and have made the code publicly available to ensure reproducibility.

==> Sensitivity_analysis.tex <==
With the goal of understanding the sensitivity of the model to the choice of the function of $\mu_\alpha(X)$ \eqref{eqn: eta}---i.e. the mean of the variable $\alpha$ involved in the weights of the mixture model---we have also estimated the model defining, for the four settings reported in Section~\ref{sec:sim}, we have also estimated the model defining using the following definition of $\mu_\alpha(X)$.

Let  $q_0 = min(x)$, $q_6= max(x)$, and $q_v$ be $v$-th observed 6-quantiles cutpoints of $X$ where  $v = 1, \dots, 5$. We  assume
 \begin{equation}\label{eqn: eta}
  \alpha_k(x) = \eta_{0,k} + \eta_{v,k}x \;\mbox{ for } x \in [q_{v-1},q_v)
 \end{equation}
where $\eta_{0,k}$ and $\eta_{v,k}$, for $v = 1, \dots, 3$, are distributed as $\mathcal{N}(\mu_{\eta},1)$.

Figure~\ref{fig:results_6quantiles} reports the comparison between the true CERF and the estimated CERF: median posterior and credible intervals.

The posterior CERFs for the four scenarios in Figure~\ref{fig:results_6quantiles} have similar behavior to the posterior CERFs in Figure~\ref{fig:results_4quantiles} in Section~\ref{sec:sim}. However, the estimation of  CERFs is still poor at the tails of the $X$, in particular for the right tail in Scenario 1 and Scenario 2 and the left tail in Scenario 4, where the $95\%$ credible interval does not include the true CERF.


\begin{figure}
\begin{center}
\includegraphics[width=2.7in]{plots_simulations/plot_c1_6q.pdf}\;\includegraphics[width=2.7in]{plots_simulations/plot_c2_6q.pdf}\\
\includegraphics[width=2.7in]{plots_simulations/plot_c3_6q.pdf}\;\includegraphics[width=2.7in]{plots_simulations/plot_c4_6q.pdf}
\end{center}
\caption{Comparison of the estimated CERF (the continuous blue line) with credible intervals---C.I.---(colored area: from dark blue for 0$\%$ to light blue $95\%$) and the true CERF (the continuous red line). \label{fig:results_6quantiles}}
\end{figure}

==> Simulations.tex <==

In this section, we present a simulation study to illustrate that our method can accurately recover the true shape of the CERF in the presence of an unmeasured confounder.

We consider four different data-generating mechanisms to evaluate the performance of our method under different scenarios. For each scenario, we generate 300 samples with a sample size equal to N=5000.

Under each of the four scenarios, we generate $U$, $W\mid U$, and $Z|U$ in the same way. More specifically, for each unit $i=1,\dots, N$, we simulate: 1)  $U_i \sim \mathcal{N}(1,0.2)$; 2) $W_i \mid U_i \sim \mathcal{N}(1-2\cdot U_i,0.2)$; and 3) $Z_i\mid U_i \sim\mathcal{N}(-1+1.5\cdot U_i,0.2)$, where $\mathcal{N}(\mu, \sigma^2)$ represents a Gaussian random variable with mean $\mu$ and variance $\sigma^2$. The four scenarios differ based on the data-generating mechanism of $Y\mid X, U$ and $X\mid U$. 
\begin{itemize}
    \item  {\bf Scenario 1}, we assume that the true distribution of the outcome $Y$ is a mixture of two linear normal regressions:
\[
    Y_i \sim \mathbb{I}_{\{X_i<5.5\}}\cdot \mathcal{N}(1+2\cdot X_i+2\cdot U_i, 0.3)+\mathbb{I}_{\{X_i\geq 5.5\}}\cdot \mathcal{N}(-16+5\cdot X_i+2.5\cdot U_i, 0.3),
\]
where $\mathbb{I}_{\{X \in \mathcal{A}\}}$ is a indicator variable such that is equal to $1$ if the realisation of the random variable $X$ belongs to the interval $\mathcal{A}$, and $0$ otherwise. We assume $X_i \mid U_i \sim \mathcal{N}(1.5+4\cdot U_i,0.2)$.


\item {\bf Scenario 2}, we assume that the true distribution of the outcome $Y$ is a parabola---i.e. the outcome is a second-order regression function of the treatment:
\[
    Y_i \sim \mathcal{N}(-10+2.2\cdot(X_i-6)^2+4\cdot U_i,0.2).
\]
We assume $X_i \sim \mathcal{N}(1.5+4\cdot U_i,0.2)$


\item {\bf Scenario 3}, we assume that the true distribution of the outcome $Y$ has a sigmoidal shape:
\[
    Y_i \sim \mathcal{N}(1.5+sign(X_i-5)\cdot\sqrt{|X_i-5|}+1.7\cdot U_i,0.05),
\]  
where $sign(a)$ is the sign function, such that is equal to $+1$ when $a\geq 0$ and equal to $-1$ otherwise. We assume  $X_i \sim \mathcal{N}(1+4\cdot U_i,0.2)$ and

\item {\bf Scenario 4}, we assume that the true distribution of the outcome $Y$ is  monotonically increasing with non-linear relation between the outcome and both the variables $X$ and $U$---treatment and unmeasured confounder, respectively:
\[
    Y_i \sim \mathcal{N}(-2\cdot e^{-1.4\cdot (X_i-6)}+0.8\cdot e^{U_i},0.2).
\]
We $X_i \sim \mathcal{N}(2.5+4\cdot U_i,0.2)$ .
\end{itemize}


For each of these four scenarios, the CERF is obtained by integrating out the unmeasured confounder $U$ in the non-linear regression for the outcome $Y\mid U, X$. Figure~\ref{fig:simulations} shows the shape of the true CERF under the four scenarios. 

\begin{figure}
\begin{center}
\includegraphics[width=2.2in]{plots_simulations/sim_1.pdf}\,\includegraphics[width=2.2in]{plots_simulations/sim_2.pdf}\\
\includegraphics[width=2.2in]{plots_simulations/sim_3.pdf}\,\includegraphics[width=2.2in]{plots_simulations/sim_4.pdf}
\end{center}
\caption{The four scenarios of the simulated  nonlinear CERF. \label{fig:simulations}}
\end{figure}

Our goal is to apply our method described in the previous section to recover the true CERFs  when we do not observe $U$. To do so, and for each unit $i$, we define the weights of the proposed nonparametric model in \eqref{eq:wights} as
\begin{equation}
    \upsilon_k(X)=\Phi(\eta_{0k}+\Tilde{X_i}^T\cdot {\boldsymbol\eta}_k)
\end{equation}
where ${\boldsymbol\eta}_k=\{\eta_{kp}\}_{p=0,1,\dots,4}$ are the weights-specific parameters, for $k\geq 1$, and $\Tilde{X_i}$ is a vector of four dummy variables defined as 
\[
    \Tilde{X_{ip}}=X_i \cdot \mathbb{I}_{\{x_i \in [q_{p-1},q_p)\}}, \mbox{    for } p=1,\dots,4;
\]
where $\mathbb{I}_{\{\cdot\}}$ is a indicator variable and $q_p$ is the $p$-th quartile, such that $\Tilde{X_{ip}}$ is equal to $X_i$ if the realisation of the variable $X_i$ belong to the interval, in the treatment support $\mathcal{S}_X$, from the $(p-1)$-th quartile (excluded) to the $p$-th quartile (included), and equal to $0$ otherwise.
In the Section~\ref{sec:app_sim}, in the Supplementary Material, we re-analyse the four scenarios defining the vector of dummy variables $\Tilde{X}_{i}$ as six variable such that $q_p$ indicate the $p$-th quantile, for each $i$. Where we show that the results using six quantiles are not different from the case illustrate in this section, using the four quartiles.  

In Figure~\ref{fig:results_4quantiles}, we show the results.  Under each scenario, the darker blue line is the median across the 300 samples of the posterior estimate of the CERF. The red line is the true CERF which is also reported in Figure~\ref{fig:simulations}. A nice feature of our method is its ability to estimate the posterior uncertainty in the estimate CERF. More specifically, with the lighter blue we report the $90\%,95\%$, and $75 \%$ posterior intervals.  We found the red curve included in the intervals, with the exception of right tail in Scenario 2 and the left tail in Scenario 4, due to the few units that we have in that tails. 

These simulation studies show that the proposed method is very flexible in a different setting and, consequently, for different shapes of the CERF.

\begin{figure}
\begin{center}
\includegraphics[width=2.6in]{plots_simulations/plot_c1_4q_smooth_02.pdf}\;\includegraphics[width=2.6in]{plots_simulations/plot_c2_4q_smooth_02.pdf}\\
\includegraphics[width=2.6in]{plots_simulations/plot_c3_4q_smooth.pdf}\;\includegraphics[width=2.6in]{plots_simulations/plot_c4_4q_smooth_02.pdf}
\end{center}
\caption{Comparison of the expected value of the CERF---in blue, with band of variability---and the simulated  nonlinear CERF---red lines. \label{fig:results_4quantiles}}
\end{figure}
